ShadowMaskFormer: Mask Augmented Patch Embeddings for Shadow Removal

Transformer recently emerged as the de facto model for computer vision tasks and has also been successfully applied to shadow removal. However, these existing methods heavily rely on intricate modifications to the attention mechanisms within the transformer blocks while using a generic patch embedding. As a result, it often leads to complex architectural designs requiring additional computation resources. In this work, we aim to explore the efficacy of incorporating shadow information within the early processing stage. Accordingly, we propose a transformer-based framework with a novel patch embedding that is tailored for shadow removal, dubbed ShadowMaskFormer. Specifically, we present a simple and effective mask-augmented patch embedding to integrate shadow information and promote the model's emphasis on acquiring knowledge for shadow regions. Extensive experiments conducted on the ISTD, ISTD+, and SRD benchmark datasets demonstrate the efficacy of our method against state-of-the-art approaches while using fewer model parameters.g fewer model parameters. Our implementation is available at https://github.com/lizhh268/ShadowMaskFormer.

==> 7-app.tex <==
\section*{Appendix}
In this supplementary material, we include: more details on the physical models of shadow removal in Section~\ref{sec:Pre}.
%
According to the original expression of shadow model~\ref{eqs1}, for a real shadow scene, an occluder blocks the direct illumination $L^d$ and part of the ambient illumination $L^a$, thus the shadowed pixel can be represented as:
\begin{equation}
\begin{aligned}
    I^{shadow}_x(\lambda) = a_x(\lambda)L^a_x(\lambda)R_x(\lambda)
\end{aligned}
\label{eqs2}
\end{equation}
where $a_x(\lambda)$ is the attenuation factor indicating the remaining fraction of $L^a$ that arrives at an image point $x$.

From these Equations, the shadow-free pixel can also be expressed as follows:
\begin{equation}\small
\begin{aligned}
    I^{shadow-free}_x(\lambda) = L^d_x(\lambda)R_x(\lambda) + a_x(\lambda)^{-1}I^{shadow}_x(\lambda)
\end{aligned}
\label{eqs3}
\end{equation}

Finally, we can express the color intensity of the lit pixel as a linear function of its shadowed value just like the expression of our paper~\ref{eq-linear}:

\begin{equation}
\begin{aligned}
    {I}_{x}^{shadow-free}(k) = w(k) \times {I}_{x}^{shadow}(k) + b_k
\end{aligned}
\label{eq-linear}
\end{equation}

